Simple subvector inference on sharp identified set in affine models

This paper studies a regularized support function estimator for bounds on components of the parameter vector in the case in which the identified set is a polygon. The proposed regularized estimator has three important properties: (i) it has a uniform asymptotic Gaussian limit in the presence of flat faces in the absence of redundant (or overidentifying) constraints (or vice versa); (ii) the bias from regularization does not enter the first-order limiting distribution; (iii) the estimator remains consistent for sharp (non-enlarged) identified set for the individual components even in the non-regualar case. These properties are used to construct \emph{uniformly valid} confidence sets for an element $\theta_{1}$ of a parameter vector $\theta\in\mathbb{R}^{d}$ that is partially identified by affine moment equality and inequality conditions. The proposed confidence sets can be computed as a solution to a small number of linear and convex quadratic programs, leading to a substantial decrease in computation time and guarantees a global optimum. As a result, the method provides a uniformly valid inference in applications in which the dimension of the parameter space, $d$, and the number of inequalities, $k$, were previously computationally unfeasible ($d,k=100$). The proposed approach can be extended to construct confidence sets for intersection bounds, to construct joint polygon-shaped confidence sets for multiple components of $\theta$, and to find the set of solutions to a linear program. Inference for coefficients in the linear IV regression model with an interval outcome is used as an illustrative example.

==> Examples/FH.tex <==

FH provide an alternative CI for $\theta_{1}$ in the affine moment
inequality model under set identification. To cover $\theta_{1}$
with probability at least $1-\alpha$ FH proposed $\mbox{CI}_{\alpha,n}^{FH}$
, an intersection of one-sided bootstrap CIs, which is analogous to
$\mbox{CI}_{\alpha,n}$.\footnote{See Section 3.3 of \citet{Freyberger201541}. FH also proposed a CI
for $\setMarginal$. One can use the joint asymptotic Gaussian distribution
of $\hat{\underline{v}}_{n}$ and $\hat{\bar{v}}_{n}$ to construct
an analogous Delta-method CI for $\setMarginal$, which can be shorter
than $\mbox{CI}_{\alpha,n}^{B}$. } In general, with probability approaching one $\left|\mbox{CI}_{\alpha,n}\right|,$
the length of $\mbox{CI}_{\alpha,n}$, is not longer than $\left|\mbox{CI}_{\alpha,n}^{FH}\right|$,
the length of $\mbox{CI}_{\alpha,n}^{FH}$, as the following proposition
shows. 
\begin{prop}
\label{prop:FH}Suppose that Assumptions \ref{assu:IID}\textendash \ref{assu:Variance}
hold. For any sequences $\mu_{n}$ and $\kappa_{n}$ such that $\kappa_{n}\to0$,
$\mu_{n}/\kappa_{n}\to0$ and $\mu_{n}\sqrt{n}\to\infty$,
\[
\lim_{n\to\infty}\measTrue\left(\left|\mbox{CI}_{\alpha,n}^{FH}\right|\geq\left|\mbox{CI}_{\alpha,n}\right|\right)=1.
\]
\end{prop}
\begin{proof}
See Appendix \ref{sec:Proof-of-Prop1}.
\end{proof}

\todo{put it in the appendix or drop}
The following example shows that $\mbox{CI}_{\alpha,n}$ can be shorter
than $\mbox{CI}_{\alpha,n}^{FH}$ in large samples.
\begin{example}
Consider the system (\ref{eq:GenericMomentConditions}) with $\Ieq=\emptyset$
and coefficients $\Data$ that have expectation
\[
\expect\Data=\left(\begin{array}{cc}
-\I[2] & - {\iota}_{2}\\
\I[2] & - {\iota}_{2}
\end{array}\right).
\]
Suppose that all components of $\Data$ are independent random
variables with variance $s^{2}$. The identified set is $\setID=\left[-1,1\right]^{2}.$
The standard deviation of every moment condition is given by $s\sqrt{1+\ltwo{ {\theta}}^{2}}$.
The asymptotic behavior of $\mbox{CI}_{\alpha,n}^{FH}$ depends on
the asymptotic distribution of the basic solutions to (\ref{prog:minP}).\footnote{See Section 3 in \citet{Freyberger201541} for details. }
The \emph{minimization} problem (\ref{prog:minP}) has two basic solutions,
$\left(-1,1\right)$ and $\left(-1,-1\right)$. The basic solutions
for the \emph{maximization} problem in (\ref{prog:minP}) are $\left(1,1\right)$
and $\left(1,-1\right)$. The critical value $c_{1-\alpha}^{FH}$
corresponds to the maximum of the $1-\alpha$ quantiles of the four
basic solutions\footnote{See Section 3.3 in \citet{Freyberger201541} for details. },
\[
c_{1-\alpha}^{FH}=z_{1-\alpha}s\max_{\theta_{1}=\pm1,\theta_{2}=\pm1}\left\{ \sqrt{1+\ltwo{\theta}^{2}}\right\} =z_{1-\alpha}s\sqrt{3}.
\]
The solution to (\ref{prog:minSSAregularized}) and to the upper bound
counterpart converge to the optima of (\ref{prog:minP}) with the
minimal norm\footnote{See Lemma \ref{lem:DeltaMethod}. }, i.e.
\begin{align*}
\funLArgHat[\mu_{n}][][\prime] & \pTo\left(-1,0\right),\\
\funUArgHat[\mu_{n}][][\prime] & \pTo\left(1,0\right).
\end{align*}
So the critical values for both sides of $\mbox{CI}_{\alpha,n}$ are
$z_{1-\alpha}s\sqrt{2}$ which leads\footnote{See Appendix \ref{sec:Proof-of-Prop1} for details}
to 
\[
\left|\mbox{CI}_{\alpha,n}^{FH}\right|-\left|\mbox{CI}_{\alpha,n}\right|=2z_{1-\alpha}s\left(\sqrt{3}-\sqrt{2}\right)n^{-1/2}+o_{p}\left(n^{-1/2}\right).
\]
As sample size grows, $\mbox{CI}_{\alpha,n}$ becomes shorter than
$\mbox{CI}_{\alpha,n}^{FH}$ with probability approaching 1,
\[
\lim_{n\to\infty}\measTrue\left(\left|\mbox{CI}_{\alpha,n}^{FH}\right|>\left|\mbox{CI}_{\alpha,n}\right|\right)=1.\QEBA
\]
\end{example}




==> Figures/Figures/Example/IDset.tex <==
\begin{figure}[H]
\begin{centering}
\begin{tabular}{ccc}
\includegraphics[scale=0.5,trim={2cm 0 1cm 0 }]{Figures/Example/RhoNegative.pdf}& \includegraphics[scale=0.5,trim={2cm 0 1cm 0 }]{Figures/Example/RhoZero.pdf}& \includegraphics[scale=0.5,trim={2cm 0 1cm 0 }]{Figures/Example/RhoPositive.pdf}\tabularnewline
\end{tabular}
\par\end{centering}
\caption{\label{fig:Identified-sets-Example2}The identified sets in Example~\ref{exa:runningExample}  for various values of $\rho$.}
\end{figure}


==> Macros/shortcutNotation.tex <==
\renewcommand{\funLLagrange}{\argminL_{\mu_n} }
\renewcommand{\funLLagrangeHat}{\hat{\argminL}_{\mu_n}}
\renewcommand{\funLArg}{\argminT_{\mu_n}}
\renewcommand{\funLArgHat}{\hat{\argminT}_{\mu_n}}

\renewcommand{\funLStd}{{\argminS}_{\mu_n}}
\renewcommand{\funLStdHat}{\hat{\argminS}_{\mu_n}}




==> Proofs/backups/DeltaMethod.tex <==
\begin{align*}
\Cov(\theta)\bydef & \expect\left[\matsq{\momentVec{\Data}{\theta}}\right]- \matsq{\MomentVec{\theta}{\measTrue}},\\
\funCovHat{\theta}\bydef & \sMean{\matsq{\momentVec{\data_i}{\theta}}}- \matsq{\sMean{\momentVec{\data_i}{\theta}}}.
\end{align*}
\todo{add shortcuts explicitly}{}
Throughout the proof of the following lemma I will suppress the argument $\measTrue$. I am also going to use a shortcut notation for {
\renewcommand{\funLLagrange}{\argminL^{\mu_n} }
\renewcommand{\funLLagrangeHat}{\hat{\argminL}^{\mu_n}}
\renewcommand{\funLArg}{\argminT^{\mu_n}}
\renewcommand{\funLArgHat}{\hat{\argminT}^{\mu_n}}



\begin{lem}
\label{lem:DeltaMethod}Consider any sequence $\mu_{n}$ such that
$\mu_{n}\to0$ and $\mu_{n}\sqrt{n}\to\infty$. Let $\measTrue$ satisfy Assumptions \ref{assu:IID}-\ref{assu:Variance} , then \todo{fix semicolon in v}{}
\begin{align*}
\sqrt{n}\frac{\funLValHat[\mu_{n}]-\funLVal[\mu_{n}]}{\funLStdHat[\mu_{n}]} & \wTo N\left(0,1\right).
\end{align*}

\end{lem}
\begin{proof}


By the  triangular inequality, \begin{eqnarray*}
\left|\trns{\funLLagrangeHat}\funCovHat{\funLArgHat}\funLLagrangeHat-\trns{\funLLagrange}\Cov(\funLArg)\funLLagrange\right| & \leq&\\
\left|\trns{\funLLagrangeHat}\funCovHat{\funLArgHat}\funLLagrangeHat-\trns{\funLLagrange}\funCovHat{\funLArg}\funLLagrange\right|&+&
\left|\trns{\funLLagrange}\funCovHat{\funLArg}\funLLagrange-\trns{\funLLagrange}\Cov(\funLArg)\funLLagrange\right|
\end{eqnarray*}
Consider $t=1/\sqrt{n}$ and 

\begin{equation}
 {\delta}\left( {\theta}\right)=\empProc{\momentVec{\data_i}{\theta}-\MomentVec{\theta}{\measTrue}}.\label{eq:deltaCLT}
\end{equation}
 By Lemma \ref{lem:CLTandLLN} $\ltwo{ \empProc{\data_i - \expect{W}}}=O_{\mathcal{P}}\left(1\right)$
uniformly in $\measTrue\in\mathcal{P}$ . I use $O_{\mathcal{P}}\left(1\right)$
to denote a random variable with a second moment uniformly bounded
over $\measTrue\in\mathcal{P}$, i.e. 
\[
\expect\ltwo{ \empProc{\data_i - \expect{W}}}^{2}\leq k\left(d+1\right)\bar{M}^{1/\left(1+\varepsilon/2\right)}.
\]
By Lemma \ref{lem:CLTandLLN} the Lipschitz constant and the Maximum
norm for $\funCovHat{\theta}$ on $\Theta$ converge in probability to the
corresponding constants of $\funCov$. 

By Lemma \ref{lem:compactPbar} the function $\eta\left(\measTrue\right)$
is bounded from below by $\eta>0.$ I can replace $\eta\left(\measTrue\right)$
in Lemma \ref{lem:2ndorderPert} by $\eta.$ By Lemma \ref{lem:2ndorderPert}
the following inequality holds for any $\mu$ if $n$ large enough, 

\begin{align*}
\left|\trns{\funLLagrangeHat}\funCovHat{\funLArgHat}\funLLagrangeHat-\trns{\funLLagrange}\funCovHat{\funLArg}\funLLagrange\right| & =\frac{1}{\mu\sqrt{n}}O_{\mathcal{P}}\left(1\right).
\end{align*}

By the triangular inequality and Lemma (\ref{lem:CLTandLLN}), 

\begin{eqnarray}
\left|\trns{\funLLagrange}\funCovHat{\funLArg}\funLLagrange-\trns{\funLLagrange}\Cov(\funLArg)\funLLagrange\right| & <\label{eq:LipschitzDelta1-1}\\
\left\Vert \funLLagrange\right\Vert _{2}^{2}\left|\left(\text{\ensuremath{\expect[\measEmp]}}-\text{\ensuremath{\expect}}\right)\left(\Data\left(\trns{\funLArg},1\right)^{\prime}\left(\funLArg,1\right)\Data^{\prime}\right)\right|+\\
\left\Vert \funLLagrange\right\Vert _{2}^{2}\left|\left(\left(\text{\ensuremath{\expect[\measEmp]}}-\text{\ensuremath{\expect}}\right)\Data\left(\trns{\funLArg},1\right)^{\prime}\left(\funLArg,1\right)\text{\ensuremath{\expect}}\Data^{\prime}\right)\right|+\\
\left\Vert \funLLagrange\right\Vert _{2}^{2}\left|\left(\text{\ensuremath{\expect[\measEmp]}}\Data\left(\trns{\funLArg},1\right)^{\prime}\left(\funLArg,1\right)\left(\text{\ensuremath{\expect[\measEmp]}}-\text{\ensuremath{\expect}}\right)\Data^{\prime}\right)\right| & = & \frac{1}{\sqrt{n}}O_{\mathcal{P}}\left(1\right),
\end{eqnarray}
where $\text{\ensuremath{\expect[\measEmp]}}\left[\cdot\right]=\sMean{\left[\cdot\right]}$.
Finally, 
\begin{eqnarray}
\trns{\funLLagrangeHat}\funCovHat{\funLArgHat}\funLLagrangeHat & = & \trns{\funLLagrange}\Cov(\funLArg)\funLLagrange+\frac{1}{\mu\sqrt{n}}O_{p}\left(1\right).\label{eq:convergenceSpeedStd}
\end{eqnarray}

\noun{Step 2.} The compact correspondences $\funLStd[][][2]$ and
$\funUStd[][][2]$ can be multivalued for $\mu=0$. The matrix function
$\funCov[\cdot]$ is continuous. By Lemma \ref{lem:continuityInMuP},
$\funLArg$, $\funUArg$, $\funLLagrange$, and $\funULagrange$ are
upper hemicontinuous for $\mu\geq0$ and continuous for $\mu>0$.
So $\funLStd[][][2],$ $\funUStd[][][2]$ are continuous for $\mu>0$.
So for any converging sequence $\left\{ \left(\mu_{n},\measTrue_{n}\right)\right\} _{n=1}^{\infty}\subset\left[0,+\infty\right)\times\mathcal{\mathcal{P}}$
with $\mu_{n}\to0$ the limits $\lim_{n\to\infty}\funLStd[\mu_{n}][\measTrue_{n}][2]$
and $\lim_{n\to\infty}\funUStd[\mu_{n}][\measTrue_{n}][2]$ exist
and belong correspondingly to the sets $\funLStd[0][\lim_{n\to\infty}\measTrue_{n}][2]$
and $\funUStd[0][\lim_{n\to\infty}\measTrue_{n}][2].$ The limits
$\lim_{n\to\infty}\funLStd[\mu_{n}][\measTrue_{n}][2]$, $\lim_{n\to\infty}\funUStd[\mu_{n}][\measTrue_{n}][2]$
are positive by Condition 5 of Definition \ref{def:-DistributionClass}.
Correspondingly by Step 1 for any $\xi>0$ ,
\begin{eqnarray}
\lim_{n\to\infty}\sup_{\measTrue\in\mathcal{P}}\measTrue\left(\funLStdHat[\mu_{n}][][2]\leq\sigma_{0}^{2}-\xi\right) & = & 0,\label{eq:stdConvergence-1}\\
\lim_{n\to\infty}\sup_{\measTrue\in\mathcal{P}}\measTrue\left(\funUStdHat[\mu_{n}][][2]\leq\sigma_{0}^{2}-\xi\right) & = & 0.
\end{eqnarray}

\noun{Step 3.} Consider any converging sequence $\left\{ \left(\mu_{n},\measTrue_{n}\right)\right\} _{n=1}^{\infty}\subset\left[0,+\infty\right)\times\mathcal{\mathcal{P}}$
with $\mu_{n}\to0$. By continuity of $\funLLagrange$ and u.h.c of
$\funLArg$ established in Lemma (\ref{lem:continuityInMuP}),
\[
\frac{\funLLagrange[\mu_{n}][\measSec][\prime]\left(\sqrt{n}\left(\sMean{  X}-\expect[\measSec]  X\right)\funLArg[\mu_{n}][\measSec]+\sqrt{n}\left(\sMean{  w}-\expect[\measSec]  w\right)\right)}{\lim_{n\to\infty}\funLStd[\mu_{n}][\measTrue_{n}][2]}\wTo N\left(0,1\right).
\]
By Slutsky's theorem, 

\[
\underline{G}_{n}\left(\mu_{n};\measTrue\right)=\frac{\funLLagrange[\mu_{n}][][\prime]\left(\sqrt{n}\left(\sMean{  X}-\expect[\measTrue]  X\right)\funLArg[\mu_{n}]+\sqrt{n}\left(\sMean{  w}-\expect[\measTrue]  w\right)\right)}{\funLStdHat[\mu_{n}]}\wTo N\left(0,1\right)
\]
uniformly in $\measTrue\in\mathcal{P}$.

By Lemma \ref{lem:2ndorderPert} the following inequality 
\[
\left|\funLValP-\funLVal+t\trns{\funLLagrange} {\delta}\left(\funLArg\right)\right|\leq t^{2}C_{v}\left(\mu,\delta\right),
\]
holds for $t$ small enough. Take $t=1/\sqrt{n}$ and $ {\delta}\left( {\theta}\right)$
as in (\ref{eq:deltaCLT}). For any realization of (\ref{eq:deltaCLT})
the following result holds
\begin{align}
\left|\sqrt{n}\frac{\left(\funLValHat[\mu_{n}]-\funLVal[\mu_{n}][\measSec]\right)}{\funLStdHat[\mu_{n}]}-\underline{G}_{n}\left(\mu_{n};\measSec\right)\right| & =\label{eq:convergence in law}\\
=\frac{\ltwo{\sqrt{n}\left(\sMean{  X}-\expect[\measSec]  X\right)}^{2}}{\mu_{n}\sqrt{n}\funLStdHat[\mu_{n}]}O\left(1\right)+\frac{\ltwo{\left(\sMean{\Data}-\expect[\measSec]\Data\right)}^{2}}{\funLStdHat[\mu_{n}]}O\left(1\right)
\end{align}
for a sufficiently large $n$ with probability approaching 1. By
Lemma \ref{lem:CLTandLLN} and \ref{eq:stdConvergence-1} the r.h.s.
of (\ref{eq:convergence in law}) converges to 0 in probability uniformly
in $\measTrue\in\mathcal{P}$ if $\mu_{n}\sqrt{n}\to\infty$. So 

\begin{equation}
\sqrt{n}\frac{\left(\funLValHat[\mu_{n}]-\funLVal[\mu_{n}]\right)}{\funLStdHat[\mu_{n}]}\wTo N\left(0,1\right)\label{eq:CLT}
\end{equation}
uniformly in $\measTrue\in\text{\ensuremath{\mathcal{P}}}$. The proof
for the upper bound is analogous. 

The proof for a fixed $\measTrue$ is analogous. The only difference
is (\ref{eq:stdConvergence-1}) is need to be replaced by
\begin{eqnarray}
\funLStdHat[\mu_{n}][][2]\pTo & \funLStd[0+][][2]> & 0,\label{eq:stdConvergence-1-1}\\
\funLStdHat[\mu_{n}][][2]\pTo & \funUStd[0+][][2]> & 0.
\end{eqnarray}



\end{proof}
} %renew commands


==> Proofs/backups/DeltaMethodPW.tex <==
 


\begin{lem}
\label{lem:DeltaMethodPW} Let $\bar{P}$ be the class of distributions satisfying Assumptions~\reF{assu:Non--empty}-\reF{assu:Moments}for any 
\begin{equation}
\lim_{n\to\infty}\sup_{\measTrue \in \mathcal{\bar{P}}}\pi(\sqrt{n}(\funLValHat[\mu_{n}]-\funLVal[\mu_{n}]),N\left(0,\funLStd[\mu_{n}][\measTrue][2]\right) )  =0.\label{eq:deltaMethodPW}
\end{equation}
\end{lem}
\begin{prooF}{lem:DeltaMethodPW}

By Lemma~\reF{lem:continuityInMu}, $\funLArg$ and $\funLLagrange$ are continuous for $\mu>0$. The matrix function $\funCov[\theta]$ is continuous in $\theta$ and thus  $\argminS\mP$ is continuous in $\mu$ for $\mu>0$. So the limit  $\lim_{n\to\infty}\funLStd[\mu_{n}][\measTrue][2]$  exists and belongs to the set $\funLStd[0][\measTrue][2]$ which by  Assumption~\reF{assu:Variance}  implies  $\lim_{n\to\infty}\funLStd[\mu_{n}][\measTrue][2]\geq\sigma_{0}^{2}$.
Result \eqref{eq:deltaMethodPW} follows immediately from \eqref{eq:convergenceSpeedStd} in Lemma~\reF{lem:consistency} , \eqref{eq:2ndOrdedBound},\eqref{eq:dmSlutsky} and Slutsky's theorem.
\end{prooF}
 
 






==> Proofs/backups/FCLTandULLN.tex <==
\todo{This lemma doesn't fit in the current form. I need to put uniform result separately}{}

\begin{lem}[Convergence of the empirical processes]
\label{lem:FCLTandULLN} The following results hold uniformly $\measTrue\in\mathcal{P}$
in for any combination of indices $r,\ell,j,m$
\begin{eqnarray}
\lim_{n\to\infty}\sup_{\measTrue\in\mathcal{P}}\measTrue\left(\left|\sMean{\left(W_{r,\ell}W_{j,m}\right)}-\expect\left|W_{r,\ell}W_{j,m}\right|\right|\geq\xi\right) & = & 0,\label{eq:2ndMoments}\\
\lim_{n\to\infty}\sup_{\measTrue\in\mathcal{P}}\measTrue\left(\left|\sMean{\left(W_{r,\ell}\right)}-\expect W_{r,\ell}\right|\geq\xi\right) & = & 0,\label{eq:1stMoments}\\
  G_{n}\left(\measTrue\right)=\sqrt{n}\left(\vecM\left(\sMean{\Data}\right)-\vecM\left(\expect\Data\right)\right) & \wTo & N\left(0, {\Omega}_{\measTrue}\right),\label{eq:UniformCLT}
\end{eqnarray}
where $ {\Omega}_{\measTrue}=\text{Cov}_{\measTrue}\left(\vecM\left(\Data\right)\right)$.
These results also hold for $\measTrue$ that satisfy Assumptions
\ref{assu:Moments}\&\ref{assu:IID}.
\end{lem}
\begin{proof}
\noun{}Consider any combination of indices for any combination of
indices $r,\ell,j,m$. By Step 2 in the proof of Lemma \ref{lem:compactPbar}
a class of random variables $W_{r,\ell}W_{j,m}$ with measures in
$\measTrue\in\mathcal{P}$ is uniformly integrable. The limit (\ref{eq:2ndMoments})
follows immediately from Proposition A.5.1 in\citet{van1996weak}.
The result (\ref{eq:1stMoments}) is analogous. The result (\ref{eq:UniformCLT})
follows from Proposition A.5.2.
\end{proof}

==> Proofs/backups/basicSolutions.tex <==

\begin{lem}
\label{lem:basicSolutions} There exist $R(\mathcal{P})>0$ such that for any $\measTrue \in \mathcal{P}$ and any measure $Q$ s.t. $\ltwo{\EW -\QW}<R(\mathcal{P})$ the following holds  $$\mathcal{B}(Q)\cap \mathcal{B}( \measTrue)\neq \emptyset$$  
\end{lem}

\begin{prooF}{lem:basicSolutions}

Step 1. One can show using the Maximum theorem argument of Lemma~\reF{lem:continuityInMu} that correspondence $\tilde{\argminT}(\cdot)$ such that $\tilde{\argminT}(\EW)\bydef\argminT(0,\measTrue)$ is a u.h.c. on any compact set that contains $\EW$. 
\todo{read comment here}{}
%\todo{this definition does not specify behavior of $\tilde{\argminT}(\cdot)$ on arbitrary compact set}{}

Let $j\in \setIneq$

$$S_j(w) \bydef \min_{\theta \in \tilde{\argminT}(w) } \ejRow w (\theta^\prime ,-1)^\prime  $$
 
By definition $S_j(w)\leq0$. \todo{Check conditions}{By the maximum theorem  $S_j(w)$ is a continuous function of w on any compact subset of $\R^{k(d+1)}$ containing $\EW$. }

Suppose that $S_j(\EW)<0$. Then by continuity there exist $R_j$ such that $S_j(w)<0$ if  $\ltwo{\EW -w}<R_j$  which implies that inequality j is not active either for such $w$. If $S_j(\EW)=0$ then take $R_j =1$. Take $R(\measTrue) \bydef min_{j\in\setIneq}{R_j}>0$.

Suppose that there is an element $\jSet^* \in \mathcal{B}(Q)$ that doesn't belong to $\mathcal{B}( \measTrue)$ for some $Q$ satisfying the assumptions of the theorem. Then $\jSet^*$ would have at least one element $j^*$ that does not belongs to any $\jSet \in \mathcal{B}(P)$. Thus $S_j(\EW)<0$ and we get a contradiction. 

Since $$\mathcal{B}(Q) \neq \emptyset$$  we get 
$$\mathcal{B}(Q)\cap \mathcal{B}( \measTrue)\neq \emptyset.$$

Now let's consider all P  in enlarged $\mathcal{P}$ with a unique basic solution.  $\ltwo{\EW -\QW}<R(P)$  makes a open cover of $\mathcal{P}$ by the previous lemma. So we can extract a finite subcover. Choose $R(\mathcal{P})$ equal to the smallest R/2 in the subcover.

Then for any $\measTrue \in \mathcal{P}$ and any measure $Q$ s.t. $\ltwo{\EW -\QW}<R(\mathcal{P})$ 
 $$\mathcal{B}(Q)\cap \mathcal{B}( \measTrue) = \mathcal{B}(P^*) \neq \emptyset$$ 


  

 \end{prooF}

==> Proofs/backups/compactP.tex <==

Let the set of the basic solutions be defined as follows,
$$ \mathcal{B}(\measTrue)\bydef \{ \activeSet\tP\big|  \theta\in\argminT(0,\measTrue), \card{\activeSet\tP} =d \}$$ 


\begin{lem}
\label{lem:compactP} The class $\mathcal{P}$ is compact in weak topology.
\end{lem}
\begin{proof}
The moments bound implies that $\mathcal{P}$ is tight. By continuity of the minimum eigenvalue function and the $l_2$ norm Assumptions 1-3 are satisfied for any limiting point. So 
$\mathcal{P}$ is closed.

\end{proof}

==> Proofs/backups/continuityMuP.tex <==
 
\begin{lem}[Continuity properties of the solution]
\label{lem:continuityInMuP}Under Assumption \ref{assu:Non--empty}
and \ref{assu:NoOveridentification}, the solution to (\ref{eq:KKTsystem}),
$\funLArg$, is upper hemicontinuous in $\mu$ for $\mu\geq0$ and
continuous for $\mu>0$; the functions $\funLLagrange$ and $\funLVal$
are continuous in $\mu\geq0$. Moreover, the function $\funLArg$
is upper hemicontinuous over the product space $\mathbb{R}_{+}\times\bar{\mathcal{\mathcal{P}}}$
and continuous on $\left(0,\infty\right)\times\bar{\mathcal{\mathcal{P}}}$;
$\funLLagrange$ and $\funLVal$ are continuous functions of $\left(\mu,\measTrue\right)\in\mathbb{R}_{+}\times\bar{\mathcal{\mathcal{P}}}$. 
\end{lem}
\begin{proof}
\noun{Structure of the proof. }First, I show that solution to (\ref{eq:KKTsystem})
can be represented as a solution to a continuous optimization problem
(\ref{eq:FBargmin}). Then I apply the Maximum theorem to (\ref{eq:FBargmin})
to establish hemicontinuity of $\funLArg[\cdot]$ on $\R_{+}$ for
a fixed $\measTrue$. Second, I repeat the argument for the product
topology on $\R_{+}\times\mathcal{\bar{\mathcal{\mathcal{P}}}}$ .
Finally, I use uniqueness of $\funLArg[\cdot]$ (and $\funLLagrange$)
to show their continuity for any $\mu>0$ ($\geq0$).

\noun{Step 1}. The function $\phi\left(a,b\right)\bydef\sqrt{a^{2}+b^{2}}+a-b$
has the following property (see \citet{fischer1992special} for details)
\begin{equation}
\phi\left(a,b\right)=0\mbox{ if and only if }a\leq0,b\geq0,ab=0.\label{eq:FBproperty}
\end{equation}
By Property(\ref{eq:FBproperty}), (\ref{eq:KKTsystem}) is equivalent
to 
\begin{equation}
\begin{cases}
\funLLagrangian & =0,\\
\ejRow\expect\Data\left( {\theta}^{\prime},1\right)^{\prime} & =0,\mbox{ for }j\in\setEq,\\
\phi\left(\ejRow\expect\Data\left( {\theta}^{\prime},1\right)^{\prime},\lambda_{j}\right) & =0,\mbox{ for }j\in\setIneq,
\end{cases}\label{eq:FBKKTsystem}
\end{equation}
where $\funLLagrangian\bydef\theta_{1}+\mu\ltwo{ {\theta}}^{2}+ {\lambda}^{\prime}\expect\Data\left( {\theta}^{\prime},1\right).$
Solutions to (\ref{eq:FBKKTsystem}) coincide with solutions to
\begin{equation}
\underset{ {\theta}\in\Theta, {\lambda}\in\mathbb{\R}^{k}}{\mathrm{argmin}}\left\{ \left\Vert \grad[ {\theta}]\funLLagrangian\right\Vert _{2}^{2}+\sum_{j\in\setEq}\left(\ejRow\expect\Data\left( {\theta}^{\prime},1\right)^{\prime}\right)^{2}+\sum_{j\in\setIneq}\left(\phi\left(\ejRow\expect\Data\left( {\theta}^{\prime},1\right)^{\prime},\lambda_{j}\right)\right)^{2}\right\} ,\label{eq:FBargmin}
\end{equation}

\noun{Step 2.} By Assumption \ref{assu:Non--empty} the program (\ref{eq:FBargmin})
has a minimizer. By Lemma \ref{lem:UniqueMin}, Assumption \ref{assu:NoOveridentification}
implies that $\funLLagrange[\mu]$ is unique and satisfies (\ref{eq:lagrangeNorm})
for any $\mu\geq0$. So the solution to (\ref{eq:FBargmin}) coincides
with 
\[
\underset{ {\theta}\in\Theta, {\lambda}\in\mathbb{R}^{k},\ltwo{ {\lambda}}\leq C_{\Theta}\left(\mu\right)\eta^{-1}\left(\measTrue\right)}{\mathrm{argmin}}\left\{ \left\Vert \grad[ {\theta}]\funLLagrangian\right\Vert _{2}^{2}+\sum_{j\in\setEq}\left(\ejRow\expect\Data\left( {\theta}^{\prime},1\right)^{\prime}\right)^{2}+\sum_{j\in\setIneq}\left(\phi\left(\ejRow\expect\Data\left( {\theta}^{\prime},1\right)^{\prime},\lambda_{j}\right)\right)^{2}\right\} .
\]

\begin{equation}
\underset{\boldsymbol{\theta}\in\Theta,\boldsymbol{\mathbf{\lambda}}\in\mathbb{R}^{k},,\ltwo{ {\lambda}}\leq C_{\Theta}\left(\mu\right)\eta^{-1}\left(P\right)}{\argmin}\left\{ \left\Vert \partial_{\theta}\mathcal{\underline{L}}\left(\boldsymbol{\theta},\boldsymbol{\lambda};\mu;P\right)\right\Vert _{2}^{2}+\sum_{j\in\mathbf{I}^{eq}}\left(\boldsymbol{e}_{j}^{\prime}\mathbb{E}_{P}\mathbf{W}\left(\boldsymbol{\theta}^{\prime},1\right)^{\prime}\right)^{2}+\sum_{j\in\mathbf{I}^{ineq}}\left(\phi\left(\boldsymbol{e}_{j}^{\prime}\mathbb{E}_{P}\Data\left(\boldsymbol{\theta}^{\prime},1\right)^{\prime},\lambda_{j}\right)\right)^{2}\right\} ,\label{eq:FBargmin-1}
\end{equation}

The objective function of this program is a continuous function of
$\mu$ and the domain is a compact valued continuous correspondence
in $\mu$. By the Maximum Theorem (See \citet{ok2007real}) $\funLXi=\left(\funLArg,\funLLagrange\right)$
is upper hemicontinuous function of $\mu\geq0$. 

Function $\funLVal=\eOneVec[\prime]\funLArg+\mu\left\Vert \funLArg\right\Vert ^{2}$
is a composition of upper hemicontinuous functions and hence, by Theorem
VI.2.1' from \citet{berge1963topological}, is upper hemicontiuous
in $\mu\in\mathbb{R}_{+}$. Since by definition $\funLVal$ is a single\textendash valued
function, upper hemicontinuity implies continuity in $\mu\geq0$ for
any fixed $\measTrue$. 

\noun{Step 3. }The set $\bar{\mathcal{P}}$ is compact in weak topology
by Lemma \ref{lem:compactPbar}. By Theorem V.2.2 from \citet{berge1963topological}
the set $\left[0,+\infty\right)\times\bar{\mathcal{P}}$ is a metric
space with a \emph{2-product metric}

\[
d_{2}\left(\left(\mu,\measTrue\right),\left(\nu,\measure[Q]\right)\right)=\sqrt{\left(\mu-\nu\right)^{2}+d_{\mbox{BL}}\left(\measure,\measure[Q]\right)^{2}}.
\]
By Lemma \ref{lem:UniformLagrangeBound}, $\eta\left(\measTrue\right)$
in Step 1 can be replaced by $\eta$. By \ref{eq:PNW2} and \ref{eq:PNW}
the objective function of Program (\ref{eq:FBargmin}) is continuous
in $\left(\mu,\measTrue\right)\in\left[0,+\infty\right)\times\bar{\mathcal{\mathcal{P}}}$.
By Maximum Theorem $\funLXi$ is upper hemicontinuous function of
$\left(\mu,\measure\right)\in\left[0,+\infty\right)\times\bar{\mathcal{P}}$.
Correspondingly, $\funLVal$ is continuous for any $\left(\mu,\measure\right)\in\mathbb{R}_{+}\times\mathcal{\bar{\mathcal{\mathcal{P}}}}$. 

\noun{Step 4.} By Lemma \ref{lem:UniqueMin} Program \ref{prog:regProg}
has a unique solution $\funLArg$ for any $\mu\in\left(0,\infty\right)$
so $\funLArg$ is a continuous function of $\mu>0$ and a continuous
function of $\left(\mu,\measure\right)\in\left(0,\infty\right)\times\bar{\mathcal{\mathcal{P}}}$. 

By Lemma \ref{lem:UniqueMin}, $\funLLagrange$ is single\textendash valued.
It implies that $\funLLagrange$ is a continuous function of $\mu\geq0$
for any fixed $\measTrue$ and a continuous function of $\left(\mu,\measure\right)$
over $\mathbb{R}_{+}\times\bar{\mathcal{\mathcal{P}}}$. 
\end{proof}

==> Proofs/backups/lengthComparisonFH.tex <==

\subsection{Proof of Proposition \ref{prop:FH}\label{sec:Proof-of-Prop1}}
\begin{proof}
\noun{Structure of the proof. }First I provide the asymptotic expansion
of the length for $\mbox{CI}_{\alpha,n}^{FH}$ and $\mbox{CI}_{\alpha,n}$.
Then I compare the critical values in $\mbox{CI}_{\alpha,n}^{FH}$
and $\mbox{CI}_{\alpha,n}$ with quantiles of the asymptotic distribution
of the support functions without regularization. The order of quantiles
implies the asymptotic length comparison.

Step 1. The $\mbox{CI}_{\alpha,n}^{FH}$ takes form
\begin{equation}
\left[\funLValHat[0]+n^{-1/2}\hat{\underline{c}}_{\alpha,n}^{FH},\funUValHat[0]+n^{-1/2}\hat{\bar{c}}_{1-\alpha,n}^{FH}\right].\label{eq:FHCI}
\end{equation}

By Section 4.1 of \citet{Freyberger201541} $\hat{c}_{1-\alpha,n}^{FH}\pTo c_{1-\alpha}^{FH}$.
So 
\begin{equation}
\left|\mbox{CI}_{\alpha,n}^{FH}\right|=\funUValO-\funLValO+\left(-\underline{c}_{\alpha}^{FH}+\bar{c}_{1-\alpha}^{FH}\right)n^{-1/2}+o_{p}\left(n^{-1/2}\right).\label{eq:lengthFH}
\end{equation}
By Theorem \ref{thm:MainTheorem} 
\begin{equation}
\left|\mbox{CI}_{\alpha,n}\right|=\funUValO-\funLValO+z_{1-\alpha}n^{-1/2}\left(\funLStd[0+]+\funUStd[0+]\right)+o_{p}\left(n^{-1/2}\right).\label{eq:lengthL2}
\end{equation}

Step 2. By Lemma \ref{lem:FCLTandULLN}
\[
\sqrt{n}\left(\sMean{\Data}-\expect\Data\right)\wTo  Z.
\]
By Theorem 3.5 of \citet{shapiro1991asymptotic}
\begin{align}
\sqrt{n}\left(\funLValHat[0]-\funLValO\right)\wTo & \min_{ {\theta}\in\funLArg[0]}\funLLagrangeO[][\prime]  Z\left( {\theta}^{\prime},1\right)^{\prime},\label{eq:nonRegL}\\
\sqrt{n}\left(\funUValHat[0]-\funUValO\right)\wTo & \max_{ {\theta}\in\funUArg[0]}\funULagrangeO  Z\left( {\theta}^{\prime},1\right)^{\prime}.\label{eq:nonRegU}
\end{align}
By Lemmas \ref{lem:constantTheta} and (\ref{lem:DeltaMethod}),
\begin{align*}
\sqrt{n}\left(\funLValHat[\mu_{n}]-\mu_{n}\left\Vert \funLArgHat[\kappa_{n}]\right\Vert ^{2}-\funLValO\right) & \wTo\funLLagrangeO[][\prime]  Z\left(\funLArg[\rTo][][\prime],1\right)^{\prime},\\
\sqrt{n}\left(-\funUValHat[\mu_{n}]+\mu_{n}\ltwo{\funUArgHat[\kappa_{n}]}^{2}+\funUValO\right) & \wTo\funULagrangeO  Z\left(\funUArg[\rTo],1\right)^{\prime}.
\end{align*}
Let $\underline{c}_{\alpha}$ and $\bar{c}_{1-\alpha}$ be the $\alpha$
and $1-\alpha$ quantiles of (\ref{eq:nonRegL}) and (\ref{eq:nonRegU})
correspondingly. By Section 3.3 of \citet{Freyberger201541} $\bar{c}_{1-\alpha}^{FH}\geq\bar{c}_{1-\alpha}$,
$-\underline{c}_{\alpha}^{FH}\geq-\underline{c}_{\alpha}$. Since
by Lemma \ref{lem:continuityInMuP} $\funLArg[\rTo]\in\funLArg[0]$
and $\funUArg[\rTo]\in\funUArg[0]$, 
\[
z_{1-\alpha}\funLStd[0+]\leq-\underline{c}_{\alpha}\text{ and }z_{1-\alpha}\funUStd[0+]<\bar{c}_{1-\alpha}.
\]
So
\[
-\underline{c}_{\alpha}^{FH}+\bar{c}_{1-\alpha}^{FH}\geq z_{1-\alpha}\left(\funLStd[0+]+\funUStd[0+]\right).
\]
The stochastic expansion for the difference between (\ref{eq:lengthFH})
and (\ref{eq:lengthL2}),
\[
\left|\mbox{CI}_{\alpha,n}^{FH}\right|-\left|\mbox{CI}_{\alpha,n}\right|=\left[-\underline{c}_{\alpha}^{FH}+\bar{c}_{1-\alpha}^{FH}-z_{1-\alpha}\left(\funLStd[0+]+\funUStd[0+]\right)\right]n^{-1/2}+o_{p}\left(n^{-1/2}\right),
\]
 implies the claim of the proposition.
\end{proof}

==> Proofs/backups/quadraticBoundOnLambda.tex <==
 

\begin{eqnarray*}
\eta\left(\measTrue\right) & = & \inf_{ {\theta}\in\partial\setID}\sqrt{\eig\left(\activeSet\tP\Ap\expect {X^{\prime}}\activeSet\tP^{\prime}\right)}>0,\\
C_{v}\left(\mu,\delta\right) & = & \mu\eta^{-4}\left(\measTrue\right)\left(1+\beta\right)\ltwo{\tilde{\Data}}^{2}+\mu^{-1}\ltwo{\argminL^\prime\dX}^{2},\\
C_{\Phi} & = & \eta^{-2}\left(\measTrue\right)\sqrt{1+\beta}L_{\Phi}\sqrt{\mu^{-1}C_{v}\left(\mu,\delta\right)}+\left(\eta{}^{-4}\left(\measTrue\right)\ltwo{\tilde{\Data}}+2\left(1+\beta\right)^{3/2}\eta^{-3}\left(\measTrue\right)\ltwo{\tilde{\Data}}^{2}\right)\\
\beta & = & \max\{1,\max_{ {\theta}\in\Theta}\ltwo{ {\theta}}^{2}\}\\
L_{\Phi} & \bydef & \max_{ {\theta}, {\nu}\in\Theta}\frac{\left\Vert \Phi\left( {\nu}\right)-\Phi\left( {\theta}\right)\right\Vert _{2}}{\left\Vert  {\nu}- {\theta}\right\Vert _{2}},\\
M_{\Phi} & \bydef & \max_{ {\theta}\in\Theta}\left\Vert \Phi\left( {\theta}\right)\right\Vert _{2}.
\end{eqnarray*}
 
 
\begin{lem}[Uniform error bounds]
\label{lem:2ndorderPert}Suppose that Assumptions \ref{assu:Non--empty}-\ref{assu:NoOveridentification}  hold. Then the following inequalities
hold for the solution of Program \ref{prog:regProgPerturbed} with
$\dmu=0$ and any $\mu\in\left(0,1/2\right]$: 
 
$$\left|\argminLd^\prime(t) \Phi \left(\argminTd(t)\right)\argminLd(t)-\argminL^\prime\Phi\left(\argminT\right)\argminL\right|   \leq tC_{\Phi}\left(\mu,\delta\right)$$
 
\end{lem}
\begin{proof}
  
Let $\beta=\max\{1,\max_{ {\theta}\in\Theta}\ltwo{ {\theta}}^{2}\}$.
The norm of the difference is bounded by
\begin{align}
\ltwo{\argminTd(t)-\funLArg}^{2} & =t^{2}\ltwo{\dot{\argminT}}^{2},\label{eq:ArgumentGrowthBound}\\
\left(\eta^{-2}\left(\measTrue\right)\left(1+\beta\right)\ltwo{\tilde{\Data}}^{2}+\mu^{-1}\ltwo{\argminL^\prime\dX}^{2}\right)t^{2} & \geq t^{2}\ltwo{\dot{\argminT}}^{2}\nonumber 
\end{align}

\noun{Step 2. }Consider the difference
\begin{eqnarray}
\left|\funLLagrangeP[][][][\prime]\Phi\left(\argminTd(t)\right)\funLLagrangeP-\funLLagrange\Phi\left(\argminT\right)\funLLagrange\right| & \leq\label{eq:difference}\\
\left|\funLLagrangeP[][][][\prime]\Phi\left(\argminTd(t)\right)\funLLagrangeP-\funLLagrangeP[][][][\prime]\Phi\left(\argminT\right)\funLLagrangeP\right|\nonumber \\
+\left|\funLLagrangeP[][][][\prime]\Phi\left(\argminT\right)\funLLagrangeP-\funLLagrangeP[][][][\prime]\Phi\left(\argminT\right)\funLLagrange\right|\nonumber \\
+\left|\funLLagrangeP[][][][\prime]\Phi\left(\argminT\right)\funLLagrange-\funLLagrange\Phi\left(\argminT\right)\funLLagrange\right| & \leq\nonumber \\
\eta^{-2}\left(\measTrue\right)\sqrt{1+\beta}L_{\Phi}\ltwo{\argminTd(t)-\funLArg}+2\left|\argminL^\prime\funLLagrangeD\right|M_{\Phi}t.\nonumber 
\end{eqnarray}
Using (\ref{eq:trick2}), I can obtain the bound for $\mu\in\left[0,1\right]$:
\begin{align*}
\left|\argminL^\prime\funLLagrangeD\right|\leq & \left|\argminL^\prime(\matD)^\prime\dA[][][][\dagger\prime]\matD\dX^{\prime}\funLLagrange\right|\\
 & +2\mu\left|\argminL^\prime(\matD)^\prime\left(\dA\dA^\prime\right)^{-1}\matD \dMomentVec\left(\argminT\right)\right|\\
\leq & \ltwo{\tilde{\Data}}\eta{}^{-3}\left(\measTrue\right)+2\mu\left(1+\beta\right)^{3/2}\eta{}^{-3}\left(\measTrue\right)\ltwo{\tilde{\Data}}^{2}
\end{align*}

So (\ref{eq:difference}) is bounded by 
\begin{eqnarray*}
\left|\funLLagrangeP[][][][\prime] {\Phi}\left(\argminTd(t)\right)\funLLagrangeP-\funLLagrange {\Phi}\left(\argminT\right)\funLLagrange\right| & \leq\\
\mu^{-1}\sqrt{2}\eta^{-4}\left(\measTrue\right)\left(1+\beta\right)L_{\Phi}\ltwo{\tilde{\Data}}t\\
+\eta{}^{-4}\left(\measTrue\right)\left(1+2\left(1+\beta\right)^{3/2}\eta\left(\measTrue\right)\ltwo{\tilde{\Data}}\right)\ltwo{\tilde{\Data}}t & .
\end{eqnarray*}
\end{proof}

==> Proofs/backups/selection.tex <==
\subsection{Proof of Theorem \ref{thm:selection}\label{sec:Proof-of-TheoremSelection}}
\Proof{selection}


% \begin{lem}
% \begin{align}
%  \sup_{\measTrue \in \Measures}\measTrue\left(\sqrt{n}(\ltwo{\funLArgHat[\mn]}^2-\ltwo{\funLArg[\mn]}^2)\geq R\right)\leq &\epsilon 
% \end{align}
% \end{lem}


% \begin{proof}
 
% \end{proof}
 Basic solutions corresponding to an active set of constraints $\jSet$ are defined as follows,
$$\bsJ(\measTrue)\bydef (\jMat\Ap )^{-1}(\jMat\bp ).$$
We can construct a uniformly consistent super-set estimator for all basic solutions using 
$$\Bhat\bydef \big\{ \jSet| \bsJvhat \leq \eOne \funLArgHat[\mn] + \mn \text{  and }\forall j\in \setIneq , \ejRow(\hat{A}\bsJhat-\hat{b})\leq \mn\big\} $$
 as the following theorem shows.
 
\begin{thm}
\label{thm:selection} Let $\mn\to0$ and $\mn \sqrt{n}\to\infty$. Then for any $\epsilon>0$ there exist n such that 
$$\inf_{\measTrue\in\Measures}\measTrue\{\mathcal{B}(\measTrue)\subset\Bhat \}\geq 1 - \epsilon.$$
\end{thm}
\begin{proof}
See Appendix~\ref{sec:Proof-of-TheoremSelection}
\end{proof}


Let the set of the basic solutions be defined as follows,
$$ \mathcal{B}(\measTrue)\bydef \{ \activeSet\tP\big|  \theta\in\argminT(0,\measTrue), \card{\activeSet\tP} =d \}$$ 

Let
$\bsJ(\measTrue)\bydef (\jMat\Ap )^{-1}(\jMat\bp )$ and
$$\Bhat\bydef \big\{  \jSet| \bsJvhat \leq \hat{\argminT}_1^{\mn} +\mn \text{  and }\forall j\in \setIneq , \ejRow(\hat{A}\bsJhat-\hat{b})\leq \mn\big\}$$
  
\begin{proof}
We need to show that $$\inf_{ \jSet\in\mathcal{B}(\measTrue);\measTrue\in\Measures}\measTrue  \big\{\bigcap_{j\in\setIneq}\{\ejRow(\hat{A}\bsJhat-\hat{b})\leq \mn\}\cap\{\bsJvhat \leq \hat{\argminT}_1^{\mn} +\mn \}\big\}\geq 1 - \epsilon $$

By Boole's inequality,
 $$\inf_{ \jSet\in\mathcal{B}(\measTrue);\measTrue\in\Measures}\measTrue  \big\{\bigcap_{j\in\setIneq}\{\ejRow(\hat{A}\bsJhat-\hat{b})\leq \mn\}\cap\{\bsJvhat \leq \hat{\argminT}_1^{\mn} +\mn \}\big\}\geq$$
 $$1 - \sup_{ \jSet\in\mathcal{B}(\measTrue);\measTrue\in\Measures}\measTrue \{\bsJvhat \geq \hat{\argminT}_1^{\mn} +\mn \} -  \sum_{j\in\setIneq} \sup_{ \jSet\in\mathcal{B}(\measTrue);\measTrue\in\Measures}\measTrue \{\ejRow(\hat{A}\bsJhat-\hat{b})\geq \mn\}$$
 
 
 By definition,  $\bsJv = \argminT_1(0,P)$. By Theorem~\ref{thm:consistency}
 $$ \hat{\argminT}^{\mn}_1 = \argminT_1\mnP+\mn(\ltwo{\argminT{\mnP}}^2 - \ltwo{\hat{\argminT}^{\mn}}^2) +O_\Measures(\frac{1}{ \sqrt{n}})$$
 By definition,
$$ \argminT_1\mnP\geq\argminT_1(0,\measTrue)$$
 By Theorem~\ref{thm:consistency},
$$\mn(\ltwo{\argminT{\mnP}}^2 - \ltwo{\hat{\argminT}^{\mn}}^2)=O_\Measures(\frac{1}{\sqrt{n}}).$$ 

As a corollary of Lemma~\ref{lem:CLTandLLN} we have
$\bsJvhat= \bsJv + O_\Measures (\frac{1}{\sqrt{n}})$

$\measTrue \{\bsJvhat \geq \hat{\argminT}_1^{\mn} +\mn  \}\leq \sup \measTrue \{O_\Measures (\frac{1}{\mn \sqrt{n}}) -O_\Measures(\frac{1}{\mn \sqrt{n}})\geq  1  \}\leq \frac{\epsilon}{1+\card{\setIneq}}.$ 


Step 2

Since $\bsJ$ is a solution, it is a feasible point, for any $j\in\setIneq$
$$ \ejRow(\Ap\bsJ-\bp)\leq .0$$ 
$$\measTrue \{\ejRow(\hat{A}\bsJhat-\hat{b})\geq \mn\}\leq \sup \measTrue \{O_\Measures (\frac{1}{\mn \sqrt{n}}) \geq 1\} \leq \frac{\epsilon}{1+\card{\setIneq}}. $$


Since $\mathcal{B}(\measTrue)$ is a finite set, the statement of the theorem is true. 

\end{proof}

==> Proofs/backups/tighteness.tex <==


\begin{defn}
Let $\mbox{BL}_{1}$ be the set of all real functions $f$ on $\mathbb{R}^{k\times(d+1)}$
with a norm
\[
\BL f\bydef\sup_{x\neq y;x,y\in\mathbb{R}^{k\times(d+1)}}\frac{\left|f\left(x\right)-f\left(y\right)\right|}{\ltwo{x-y}}\leq1.
\]
The \emph{bounded Lipschitz metric }for $\measure[][1],\measure[][2]\in\mathcal{P}$
is 
\[
d_{BL}\left(\measure[][1],\measure[][2]\right)=\sup_{f\in BL_{1}}\left|\int fd\measure[][1]-\int fd\measure[][2]\right|.
\]

Metric $d_{BL}\left(\measure[][1],\measure[][2]\right)$ generates
the topology of weak convergence on $\bar{\mathcal{P}}$ ( Theorem
1.12.4 \citet{van1996weak}). 
\end{defn}
\begin{lem}[Topological properties of $\mathcal{P}$ ]
\label{lem:compactPbar}  The closure of $\mathcal{P}$, $\bar{\mathcal{P}}$,
is compact in weak topology and satisfies conditions 1-4 of Definition
\ref{def:-DistributionClass}. Moreover, for any convergent sequence
$\left\{ \measure[][n]\right\} _{n=1}^{\infty}\subset\mathcal{P}$
and any combination of indices $r,\ell,j,m$
\begin{align}
\expect[\measSec]\left|W_{r,\ell}W_{j,m}\right| & \to\expect\left|W_{r,\ell}W_{j,m}\right|,\label{eq:PNW2}\\
\expect[\measSec]\Data & \to\expect\Data,\label{eq:PNW}
\end{align}
where $\measSec\wTo\measTrue.$
\end{lem}
\begin{proof}
\noun{Structure of the proof. }First I show that $\mathcal{P}$ is
uniformly tight so compactness of its closure, $\bar{\mathcal{P}}$,
follows from the Prokhorov theorem. Then I prove conditions 1-4 in
Definition \ref{def:-DistributionClass} for any limiting point of
$\mathcal{P}$ using the uniform integrability properties of $\Data$
and the corresponding continuity properties of the functions involved
in Definition \ref{def:-DistributionClass}. 

\noun{Step 1.} By Definition \ref{def:-DistributionClass} and Jensen's
inequality, for any $\measTrue\in\mathcal{P}$
\[
\expect\ltwo{\Data}^{2}\leq k\left(d+1\right)\bar{M}^{\frac{2}{2+\varepsilon}}.
\]
Consider a compact set for any positive $\xi,$
\[
\mathcal{K}^{\xi}=\left\{ \ltwo{\Data}^{2}\leq\xi k\left(d+1\right)\bar{M}^{\frac{2}{2+\varepsilon}}|\Data\in\R^{k\times\left(d+1\right)}\right\} .
\]
By Chebyshev's inequality for any $\measure\in\mathcal{P}$,
\begin{equation}
\measure\left\{ \Data\in\mathcal{K}^{\xi}\right\} >1-\frac{1}{\xi}.\label{eq:Chebyshev}
\end{equation}
 The set $\mathcal{K}^{\xi}$ does not depend on $\measure\in\mathcal{P}$,
so $\mathcal{P}$ is uniformly tight. By the Prohorov's Theorem (see
Theorem 1.3.9 in \citet{van1996weak}) the uniformly tight set $\mathcal{P}$
is a \emph{precompact} (or \emph{relatively compact}) in weak topology.
Since the $\mathcal{P}$ precompact, its closure $\bar{\mathcal{P}}$
is a sequential compact in weak topology. 

By Theorem 1.12.4 from \citet{van1996weak} the weak convergence on
$\bar{\mathcal{P}}$ is metrizable by $d_{BL}$. For a metric spaces
sequential compactness is equivalent to compactness. 

\noun{Step 2.} Consider any weakly converging sequence $\left\{ \measure[][n]\right\} _{n=1}^{\infty}\subset\mathcal{P}$
such that $\measure[][n]\wTo\measure$. By Schwarz and Jensen's inequalities,
for any combination of indices $r,\ell,j,m$
\begin{align*}
\expect[\measSec]\left|W_{r,\ell}W_{j,m}\right|^{1+\varepsilon/2} & \leq\left(\expect[\measSec]\left|W_{r,\ell}\right|^{2+2\varepsilon}\expect[\measSec]\left|W_{j,m}\right|^{2+2\varepsilon}\right)^{1/2}\leq\bar{M}.
\end{align*}
So for any $\measSec\in\mathcal{P}$ and any combination of indices
$r,\ell,j,m$ the random variables $\left|W_{r,\ell}\right|$ and
$\left|W_{r,\ell}W_{j,m}\right|$ have correspondingly finite $1+\varepsilon/2$
and $2+\varepsilon$ moments. The bound on the moments is independent
of $\measSec\in\mathcal{P}$, so these random variables with measures
$\left\{ \measSec\right\} $ are uniformly integrable (see p. 67 in
\citet{kallenberg2006foundations}). By Lemma 4.11 in \citet{kallenberg2006foundations},
the uniform integrability implies
\begin{align*}
\expect[\measSec]\left|W_{r,\ell}W_{j,m}\right| & \to\expect\left|W_{r,\ell}W_{j,m}\right|,\\
\expect[\measSec]\Data & \to\expect\Data,\\
\liminf_{n\to\infty}\expect[\measSec]\left|W_{r\ell}\right|{}^{2+\varepsilon} & \geq\expect[\measTrue]\left|W_{r\ell}\right|{}^{2+\varepsilon}.
\end{align*}
The last inequality implies that any $\measTrue\in\bar{\mathcal{P}}$
satisfies Condition 1 in Definition \ref{def:-DistributionClass}.

\noun{Step 3.} By Condition 2 of Definition \ref{def:-DistributionClass}
$\setID[\measSec]$ is not empty for every $n\in\mathbb{N}$. Pick
a point $\vartheta_{n}\in\setID[\measSec]$ for every $n\in\mathbb{N}$.
Since every $\vartheta_{n}$ belongs to the compact set $\Theta$,
there exist a convergent subsequence $\left\{ \vartheta_{n_{\ell}}\right\} _{\ell=1}^{\infty}$
. Let $\vartheta^{*}\bydef\lim_{\ell\to\infty}\vartheta_{n_{\ell}}$.
By (\ref{eq:PNW}), $\vartheta^{*}\in\setID$. So Condition 2 of Definition
\ref{def:-DistributionClass} is satisfied for any $\measTrue\in\bar{\mathcal{P}}$.

\noun{Step 4.} By Step 1, $\bar{\mathcal{P}}$ is a metric space.
By (\ref{eq:PNW}), the set $\setID$ is a compact\textendash valued
continuous correspondence at any $\measTrue\in\bar{\mathcal{P}}$.
Analogously, the objective function of Program (\ref{eq:inconsistenSystems})
is continuous in $\measTrue\in\bar{\mathcal{P}}$. It implies that
Program (\ref{eq:inconsistenSystems}) satisfies the conditions of
the Maximum Theorem (see the corresponding section in \citet{ok2007real}).
As a result, the value of Program (\ref{eq:inconsistenSystems}) is
a continuous function of $\measTrue\in\bar{\mathcal{P}}$. By this
continuity property, any $\measTrue\in\bar{\mathcal{P}}$ satisfied
Condition 3 of Definition \ref{def:-DistributionClass}. 

By continuity of $\eig\left(\cdot\right)$, any $\measTrue\in\bar{\mathcal{P}}$
also satisfies Condition 4 of \ref{def:-DistributionClass}. 
\end{proof}

==> Proofs/backups/uniformBoundOnLambda.tex <==
 
\begin{lem}[Uniform bound on Lagrange multipliers]
\label{lem:UniformLagrangeBound}  For any $\measTrue\in\mathcal{\bar{P}}$
\[
\eta\left(\measTrue\right)=\min_{ {\theta}\in\partial\setID}\sqrt{\eig\left[\left(\setIndexActive[\theta]\expect  X\expect  X^{\prime}\setIndexActive[\theta]^{\prime}\right)\right]}\geq\eta.
\]
Correspondingly,
\begin{align*}
\ltwo{\funLLagrange} & \leq\eta^{-1}C_{\Theta}\left(\mu\right),\\
C_{\Theta}\left(\mu\right)\bydef & \max_{ {\theta}\in\Theta}\ltwo{\eOneVec+2\mu {\theta}}.
\end{align*}
\end{lem}
\begin{proof}
Lemma \ref{lem:compactPbar} and Conditions 3-4 of Definition \ref{def:-DistributionClass}
imply that any $\measTrue\in\bar{\mathcal{P}}$ satisfy Assumption
(\ref{assu:NoOveridentification}). By Lemma (\ref{lem:LICQ}), any
$\measTrue\in\bar{\mathcal{P}}$ satisfies Assumption (\ref{assu:LICQ}).
Set $\setIndexActive[\theta]$ is nonempty for any $\theta\in\partial\setID$.
Assumption (\ref{assu:LICQ}) implies that for any $\theta\in\partial\setID$
\[
\eig\left[\left(\setIndexActive[\theta]\expect  X\expect  X^{\prime}\setIndexActive[\theta]^{\prime}\right)\right]>0.
\]
The Rouch\'{e}\textendash Capelli theorem implies that ranks and,
correspondingly, the numbers of the positive eigenvalues are equal
for the following matrices 
\begin{align}
\expect\left(  X,-  w\right)^{\prime}\setIndexActive[\theta]^{\prime}\setIndexActive[\theta]\expect\left(  X,-  w\right) & ,\label{eq:eigenValues2}\\
\expect  X^{\prime}\setIndexActive[\theta]^{\prime}\setIndexActive[\theta]\expect  X & .\label{eq:eigenValues}
\end{align}
Let this number be $\ell$. By the Courant\textendash Fischer\textendash Weyl
min-max principle, the $\ell$-th largest eigenvalue of (\ref{eq:eigenValues2})
can be represented as
\begin{equation}
\tau_{\ell}=\max_{U:\dim U=\ell}\left\{ \min_{ {\nu}\in U\subset\R^{d+1}} {\nu}^{\prime}\expect\left(  X,-  w\right)^{\prime}\setIndexActive[\theta]^{\prime}\setIndexActive[\theta]\expect\left(  X,-  w\right) {\nu}/\ltwo{ {\nu}}^{2}\right\} ,\label{eq:CFW1}
\end{equation}
where maximum is taken over all linear subspaces $U\subset\R^{d+1}$
with dimension $\ell$. Similarly, the $\ell$-th largest eigenvalue
of (\ref{eq:eigenValues}) can be represented as
\begin{equation}
\tilde{\tau}_{\ell}=\max_{U:\dim U=\ell}\left\{ \min_{ {\nu}\in U\subset\R^{d}} {\nu}^{\prime}\expect  X^{\prime}\setIndexActive[\theta]^{\prime}\setIndexActive[\theta]\expect  X {\nu}/\ltwo{ {\nu}}^{2}\right\} .\label{eq:CFW2}
\end{equation}
For any fixed $U$ the value of the minimization program in (\ref{eq:CFW2})
is not smaller than the corresponding value in (\ref{eq:CFW1}) since
the corresponding domains are nested. It implies $\tilde{\tau}_{\ell}\geq\tau_{\ell}$. 

Positive singular values do not change by matrix transposition operation.
By this property of singular values the matrix $\setIndexActive[\theta]\expect\left(  X,-  w\right)\expect\left(  X,-  w\right)^{\prime}\setIndexActive[\theta]^{\prime}$
has the same set of positive eigenvalues as the matrix (\ref{eq:eigenValues2}).
By Condition 4 from \ref{def:-DistributionClass} $\tau_{\ell}\geq\eta^{2}$.
Similarly, any eigenvalue of the matrix $\setIndexActive[\theta]\expect  X\expect  X^{\prime}\setIndexActive[\theta]^{\prime}$
is also an eigenvalue of (\ref{eq:eigenValues}). So 
\[
\sqrt{\eig\left[\left(\setIndexActive[\theta]\expect  X\expect  X^{\prime}\setIndexActive[\theta]^{\prime}\right)\right]}\geq\eta,
\]
and $\eta\left(\measTrue\right)\geq\eta$ for any $\measTrue\in\text{\ensuremath{\mathcal{P}}}.$
The uniform bound on $\ltwo{\funLLagrange}$ follows from Lemma \ref{lem:UniqueMin}.
\end{proof}

==> Proofs/backups/uniformMuBar.tex <==
 
\begin{lem}
\label{lem:FirstCoordinate}There exist $\mu_{1}\left(\mathcal{P}\right)>0$
such that for any $0\leq\mu\leq\mu_{1}\left(\mathcal{P}\right)$ and
$\measTrue\in\mathcal{P}$ $\eOneVec[\prime]\funLArg=\funLValO$. 
\end{lem}
\begin{proof}
Consider
\begin{equation}
\mu_{1}\left(\measTrue\right)=\max_{\eOneVec[\prime]\funLArg=\funLValO,0\leq\mu\leq1}\mu.\label{eq:mu1}
\end{equation}
By Lemma (\ref{lem:constantTheta}) for any $\measTrue\in\mathcal{P}$
and $0\leq\mu\leq\bar{\mu}\left(\measTrue\right)$ $\eOneVec[\prime]\funLArg=\funLValO$.
So $0<\min\left\{ \bar{\mu}\left(\measTrue\right),1\right\} \leq\mu_{1}\left(\measTrue\right)$.
By Lemma \ref{lem:continuityInMuP} the function $\eOneVec[\prime]\funLArg$
is continuous. The set
\[
\mathcal{D}\left(\measTrue\right)=\left\{ \mu|\eOneVec[\prime]\funLArg=\funLValO,\text{ }0\leq\mu\leq1\right\} 
\]
is a compact\textendash valued continuous correspondence for $\measTrue\in\mathcal{P}$.
By the Maximum Theorem (See \citet{ok2007real}) $\mu_{1}\left(\measTrue\right)$
is a continuous function of $\measTrue\in\mathcal{P}$. By Lemma \ref{lem:compactP}
$\mathcal{P}$ is compact so 
\[
\mu_{1}=\min_{\measTrue\in\mathcal{P}}\mu_{1}\left(\measTrue\right)>0.
\]
\end{proof}

==> Sections/Backups/ScopeDiscussion.tex <==

\subsection{Scope}

There are at least two recent papers, BCS and KMS,  to construct confidence sets that provide explicit  classes of DGP with uniform asymptotic coverage probability. 
Both methods are applicable in  non-linear moment inequality models.
They however are more restrictive in some other dimensions and there are examples of affine moment inequality models that fall outside of their scope. 

Both methods are using standardized moment conditions and hence restrict variance of the moment conditions to be strictly larger that some small constant (Definition 4.2.ii in BCS and  Assumption 4.1 b (iii) in KMS). 
Moreover, the standardized moment conditions has to be   differentiable (Assumption A.3.c in BCS and 4.4.i in KMS). 
Both Assumptions are also present in the pioneering AS paper.  
The following example illustrates violation of these assumptions in an affine models.

\begin{example}[Example 1 continued]
 Suppose that for some support point $ {  z}_{0}$ with a positive mass the lower bound on the outcome is deterministic, i.e. $\expect\left(\underline{Y}| Z= {z}_{0}\right)=y_{0}$
and $\text{Var}_{\measTrue}\left(\underline{Y}|Z= {  z}_{0}\right)=0$.
The corresponding moment inequality condition is
\begin{equation}
\expect g(Y,Z,\theta) =\expect\left[\left(\underline{Y}-  z_{0}^{\prime} {\theta}\right)\Ch{  {  Z}= {z}_{0} } \right]\leq0.\label{eq:detBound}
\end{equation}

The standard deviation of the moment condition is $\left|  z_{0}^{\prime} {\theta}-y_{0}\right|\sqrt{p_{z}\left(1-p_{z}\right)}$,
where $p_{z}=\expect\Ch{  {  z}= {  z}_{0}} $. 
It is equal to zero for any solution of the linear equation $  z_{0}^{\prime} {\theta}=y_{0}$. 
These values of $ {\theta}$ make the constraint (\ref{eq:detBound}) binding, which is exactly the case when this constraints determines $\funLValO$. 
This moment condition is also non-differentiable at these points.
\[
\partial_\theta g(y_0,z_0,\theta)=  \text{sign}\left(y_{0}-  z_{0}^{\prime} {\theta}\right)\sqrt{p_{z}/\left(1-p_{z}\right)}.\QEDB
\]
\end{example}

I also avoid imposing any restrictions on the correlation matrix of the moment conditions which is present in KMS (Assumption 4.3) and the polynomial minorant condition (Assumption A.3.a in BCS, present in CHT, avoided in KMS). 

I do impose an explicit assumptions that guarantee the LICQ which is not present in KMS or BCS, but I only require them to hold in subproblems, as noted in Section~\ref{subsec:overidentification}. 
I would like to note here that the M-step in KMS uses standard Newton optimization routines that can find all the stationary (KKT) points. 
If there is no constraint qualification, however, KKT conditions are no longer providing the necessary conditions for the optimum, which in this case is a John-Fritz conditions.\footnote{See Section 5.2.2 in \BS }
As a result, E-A-M algorithm considered in KMS is not guaranteed to converge to the global optimum without some constraint qualification.  

==> Sections/Empirics.tex <==
\section{ Outline for an Empirical Application}\label{sec:Empirics}
This section contains a potential empirical application of the proposed procedures.


==> Sections/Extension.tex <==
\section{Extensions}\label{sec:extensions}
In this section I outline how to use the regularized support function approach to construct joint confidence sets for multiple components of $\theta$ and tackle the intersection bound problem. 
The latter problem appears once we represent the value of program \eqref{prog:minP} as a maximum over values of its subproblems. 
Such subproblems may meet Assumptions~\ref{assu:RankCondition}-\ref{assu:NoOveridentification} even if the full problem does not.

 
\subsection{Dealing with overidentification \label{subsec:overidentification}}

Another interesting extension concerns the case when Assumptions~\ref{assu:Non--empty}-\ref{assu:NoOveridentification} are violated for $\setID$, but it can be represented as an intersection of sets  $s=1,...,L$, $\Theta^s(\measTrue)$   which satisfy these assumptions. Then
\begin{equation}
    \underline{v}(\measTrue)= \min_{ {\theta}\in\setID} \eOne {\theta}\geq \max_{ s=1,...,L}(\min_{ {\theta}\in\Theta^s(\measTrue)} \eOne{\theta})\geq \max_{ s=1,...,L}  \minV^{s,out}(\mu_{n},\measTrue)  \label{eq:overidentificationBound}
\end{equation}
 If we define $ \underline{v}(\measTrue)=+\infty$ in the case $\setID=\emptyset$, then the bounds \eqref{eq:overidentificationBound} are trivially valid too.

It is possible to make the first bound in \eqref{eq:overidentificationBound} sharp if we consider all subsets of $d-p$  inequality restrictions (besides the ones that define $\Theta$) as the following example shows.
\begin{example}[Example \ref{exa:runningExample} continued] 
Consider  all $L=C(K,d)=C(4,2)=6$ subsystems $\Theta^s(\measTrue)$ of \eqref{eq:fullsystem} corresponding to any two support points $z,z^\prime\in\{0,1\}^2$. 
We can get a sharp bound on $\underline{v}(\measTrue)$ in form of a maximum of the values of the subproblems,
$$\underline{v}(\measTrue)= \min_{ {\theta}\in\setID} \eOne {\theta}= \max_{ s=1,...,L}(\min_{ {\theta}\in\Theta^s(\measTrue)} \eOne{\theta}).$$
Indeed, value $\underline{v}(\measTrue)$ is attained at some basic solution $\theta^{(s)}$. 
By definition, at such $\theta^{(s)}$  at least two inequalities are active. 
There exist a subproblem $\Theta^s(\measTrue)$ that contains the same two inequalities. 
By construction, $\theta^{(s)}_1 = \min_{ {\theta}\in\Theta^s(\measTrue)} \eOne{\theta}\QEDB$.
\end{example}



Let $\minV^{(s)}$ denote the solution to the subproblem $s$.  Since every subproblem satisfies Assumptions~\ref{assu:Non--empty}- \ref{assu:NoOveridentification}, we get

$$\sqrt{n}\left(\begin{array}{c}
{\minV}^{(1)}(\mn,\measEmp) - \minV^{(1)}(\mn,\measTrue)\\
\cdots\\
{\minV}^{(L)}(\mn,\measEmp) - \minV^{(L)}(\mn,\measTrue)
\end{array}\right)\wTo N(0,\Omega).$$
As before,
$$\Omega_{ij} = \expect [\lambda^{\prime(i)}\momentVec{W}{\argminT^{(i)}} \momentVec{W}{\argminT^{(j)}}^\prime\lambda^{(j)}].$$


\begin{rem} \label{rem:specificationTest}\emph{Specification testing}
The subproblem representation \eqref{eq:overidentificationBound} can provide a test for model specification, i.e. the test of Assumption~\ref{assu:Non--empty}. 
Under the misspecification, the case  $\Theta(\measTrue)=\emptyset$, the lower bound on the minimum $\minV(\measTrue)$  is larger than the analogous upper bound on the maximum $\maxV(\measTrue)$. 
It should always be possible to find subproblems with non-empty domains and finite values in the sample, $\minV^s(\measEmp)$ and $\maxV^{s^\prime}(\measEmp)$.
The t-test of the hypothesis   $$\minV^{s,out}(\mn,\measTrue)\leq\maxV^{s^\prime,out}(\mn,\measTrue)$$ can be interpreted as a specification test. 
I leave this extension for future work.
\end{rem}




==> replyToReferees.tex <==
\newpage
\setcounter{page}{1}

\section*{Response to the Editor}

Dear Editor,

Thank you for giving me an opportunity to revise  the paper. As in the previous round, I believe that the paper benefited a lot from the revision. 
The main focus of the revision was to cut technical details on LICQ, change formating of the examples and assumptions, and do a careful proofreading. 
Below, I provide detailed point-by-point replies to all the comments of the Associate Editor and the three referees. 

\bigskip

Sincerely,

\smallskip 

  Bulat Gafarov 


 

\section*{Response to the Associate Editor}

Thanks a lot for your constructive and thoughtful comments.
I provide detailed point-by-point replies below.

 
\begin{enumerate}
    \item  \textit{\textcolor{blue}{I only want to add one additional comment. I am not convinced by Remark 2, which
argues that certain assumptions hold generically. Although the statement is correct, it is
also misleading. Full rank conditions (even in linear IV models) always hold generically, but
this does not imply that these assumptions are necessarily reasonable or nothing to worry
about. Moreover, it seems to me that uniqueness of the solution to the linear programming
problem also holds generically, which would then suggest that the proposed method might
not even be needed.}}

\smallskip

\textbf{Response:} Following your suggestion, I omit Remark 2 from the paper. Regarding generic uniqueness of solutions for linear programs. It is not generic, since for any DGP  $P$ with $d>1$ there exist multiple directions (given by   normal vectors of inequalities that define the identified set) at which the support function is not differentiable. So regularization is required to obtain valid inference uniformly over all the directions on the unit sphere.   



\end{enumerate}




 

\section*{Response to Referee 1}

Thanks a lot for your constructive and thoughtful comments. 


 \begin{enumerate}
\item[1.]
\textit{\textcolor{blue}{The author extensively discussed the LICQ. This was needed for the review process,
but the material in Section 3.1.1 is probably too much for the general reader of the
journal. After clearly stating Assumptions 4-5, I suggest the author focus on the
following points.
• Assumptions 4 and 5 are testable and are sufficient for the LICQ;
• They rule out singleton identified sets and overidentifying restrictions;
• The paper should illustrate these points clearly through examples. Using Example
3 is fine, but some of the discussion (especially the bottom half of page
13) still focuses on technical aspects. As suggested by another referee, I think
the paper should focus on explaining the practical meaning of Assumptions 4-5.
Since the paper can handle various examples, taking another empirical example
(such as that of Syrgkanis et. al., 2017) and explaining what Assumptions 4-5
rule out in that context may be a possibility.}}

 \smallskip
\textbf{Response:}

Following your suggestion, I shortened Section 3.1.1 with the focus on testability and practical implicaitons of Assumption \ref{ass:ULICQ} (former Assumptions 4-5). I omited some technical remarks and moved others to Appendix \ref{subsec:LICQdiscussion}.
Regarding practical examples, the Assumption 2 is satisfied generically for applications with non-empty sample identified set. The characteristics $s$ and $\eta$ will depend on specific dataset and thus would require various sample sizes for the procedure to work as intended. 
  
\item[2.] \textit{\textcolor{blue}{Regarding the settings that are not covered by the paper, I found the author’s response
and description in the text unsatisfactory. It is fine to claim that the paper
can cover interesting and meaningful examples. However, I think it is equally important
to be clear and upfront about what this paper does not cover. Any paper has
limitations, and this paper is making useful contributions within its scope.
Unfortunately, I did not find footnote 7 or the concluding remarks useful. It’s better to provide examples and references more clearly earlier in the text.}}
 
 \smallskip
\textbf{Response:} I added a disclaimer about the applications that are not covered by my method in the second paragraph on page 3 :

\emph{This paper focuses on the case with finitely many affine unconditional inequalities that are non-overidentifed and that result in a non-empty identified set. 
This, of course, rules out many interesting economic applications that involve overidentifying moment inequalities  \citep[for example,][]{shi2018estimating}, or where the moment inequalities are nonlinear \citep[for example,][]{pakes2015moment}. }

\item[3.] \textit{\textcolor{blue}{The paper can improve exposition further by focusing on its core contributions. Examples
of the material that can be shortened are as follows.
 Detailed discussion following Theorem 1 on the effects of $\mu_n$ and $\kappa_n$.
 Discussion on the strong approximation following Theorem 2.}}
 
 \smallskip

\textbf{Response:} Following your suggestion, I shortened the discussions after Theroem 1 and 2 in half. 

 
\item[4.] \textit{\textcolor{blue}{ The updated title and text contain the term “sharp identified set”. This term carries
a specific meaning in the partial identification literature (i.e., given available data and model assumptions, it is the smallest set of observationally equivalent parameter values consistent with the model). The paper uses a ``sharp identified set'' to mean
a non-enlarged identified set. However, the non-enlarged set characterized by affine
restrictions may or may not be sharp. To avoid confusion, it would be better to avoid
using the term ``sharp'' .}}
 
\textbf{Response:}  I take a system of inequalities (2.2) is a definition of the statistical model. For this model, I propose inference method for the smallest set of observationally equivalent parameter values consistent with the model, i.e. sharp identified set. I believe the title of the paper helps to differentiate myself from \cite{cho2023simple} who enlarges the original set by an arbitrary amount. I would like to keep the current title. 

\item[Additional comments.] 

 
\textbf{Response:}  I added definition of $W$ following the referee's suggestion and corrected the typo on Page 2. On page 7 I added replaced \emph{differentiable in the data} with \emph{differentiable in the sample mean $\sMean W_i$} to be precise.  I also highlighted that I am talking about the sample analog $\hat{\underline{v}}_n$  in that paragraph. 

 \end{enumerate}





 

\section*{Response to Referee 2}

Thanks a lot for your constructive and thoughtful comments. 
 



 \begin{enumerate}

\item[1.]   \textit{\textcolor{blue}{Please unify the notation $\mu_n$ and $\mu$, and $\kappa_n$ and $\kappa$.}}

 \smallskip

\textbf{Response:} These four tuning parameters are conceptually different from  each other. That is why I use four special symbols. I think using a separate symbol $\kappa$ is better than adding subscripts or superscripts to $\mu$.
 
After Theorem 1, I explain the difference between the fixed value $\mu$ and the shrinking sequence $\mu_n$:

\emph{So instead of trying to estimate $\bar{\mu}(\measTrue)$, I suggest using two appropriately chosen shrinking sequences $\mu_n$ and $\kappa_n$ instead of fixed tuning parameters $\mu$ and $\kappa$.}


\item[2.] \textit{\textcolor{blue}{Some comments in the footnotes are essential, and I prefer putting them in the main
context, such as Footnote 4 on Page 2, Footnote 7 on Page 4, and Footnote 11 on Page 11.}}
 
 \smallskip

\textbf{Response:} Following your suggestion, I incorporated Footnote 4 into the main text in the same paragraph.  Footnote 11 now is a new paragraph on the same page. Instead of Footnote 7, I added a disclaimer about the applications that are not covered by my method in the second paragraph on page 3 :

\emph{This paper focuses on the case with finitely many affine unconditional inequalities that are non-overidentifed and that result in a non-empty identified set. 
This, of course, rules out many interesting economic applications that involve overidentifying moment inequalities  \citep[for example,][]{shi2018estimating}, or where the moment inequalities are nonlinear \citep[for example,][]{pakes2015moment}. }

\item[3.] \textit{\textcolor{blue}{I think the examples should be reorganized. Example 2 is an empirical study of Example
1so it’s unclear why there are two examples. Moreover, Example 3 and Example 4
are continuing discussions of Example 1, so they’re the same examples too. Example 5
is about a polygonal joint confidence set, so it’s unclear why this is an example. These
all make the paper hard to read. It also gives me the impression that the linear IV
model with interval-valued outcomes is the only example the author can think of. If
not, please clarify. If yes, perhaps you can have a section about linear IV models with
interval-valued outcome and summarize all relevant results in that section.}}
 
 \smallskip

\textbf{Response:} Following your suggestion,  I renamed Section 2.2  ``Motivating example: Linear IV model  with interval-valued outcome''.    I I start this section now with the following paragraph:

\emph{ The polygon-shaped identified sets considered in this paper appear in many econometric models that feature discrete data, as mentioned in the introduction. 
Many of these applications are concerned with  instrumental variables. 
 I use the linear IV model with interval outcome  \citep[for example,][]{manski2003partial,chernozhukov2007estimation} to illustrate ideas throughout the paper. Other applications of the proposed method include monotone IV \citep{manski2000monotone}  and nonparametric IV \citep{Freyberger201541}.}

Within this section, I do not use Example environment for the former examples 1 and 2. Example 5 is now part of the main text.  So, the paper now has only one analytical Example 1  (former 3 and 4).



\item[4.] \textit{\textcolor{blue}{I also think the author should separate the discussion of theoretical results from the implementations instead of pooling them together. This also make the paper hard to
read. }}


 \smallskip

\textbf{Response:} I am not sure which section the referee has in mind. I assume, he/she meant Section 3.1.1, which  was very technical indeed.  So I shortened that section  and moved technical discussion to Appendix A. 

 \end{enumerate}


 

\section*{Response to Referee 3}

Thanks a lot for your constructive and thoughtful comments. 
 
 \begin{enumerate}
\item[1.] 
\textit{\textcolor{blue}{ The paper remains unnecessarily long to my taste. Among other things,
I would in particular only formalize an assumption only if it is needed to present the main results.}}

 \smallskip

\textbf{Response:} Slater condition and LICQ are now formulated using Condition environment. Former Assumptions 4-5 are now Assumption 2. Assumption 6 (i.i.d. data) now is stated as a part of the setup. Assumption 7 now become Assumption 3. In the current version I only have 3 assumptions left, all of which are used in the main results.  The main text of the paper got shorter by 2 pages as the result of the revision. 


\item[2.] \textit{\textcolor{blue}{ The bounds on $\underline{v}(P)$ on page 16: It would helpful to motivate why different
corrections are used in (3.11) and (3.12): one involves $\theta(\kappa, P)$ and the
other $\theta^*$. And then below Theorem \ref{thm:bounds} I would give an explanation in plain
language of what ``the regular case'' means.}}

 \smallskip

\textbf{Response:} I moved the motivation the two separate bounds are necessary for uniform one-sided inference before Theorem 1:

\emph{The expressions in \eqref{eq:innerOuterBounds} provide valid conservative bounds from above and below for $\minV(\measTrue)$ that are useful for uniform one-sided inference (coverage probability in this case can be higher than nominal level). For the remainder of the paper, the focus will be on the confidence bounds that cover $\minV (\measTrue)$ from below. So $\minVout(\mu,\measTrue) $ will play the major role. The uses of $\minVin(\mu,\kappa,\measTrue)$ for uniform inference are discussed in Appendix Section \ref{subsec:overidentification} }


I also now  say  explicitly that the nonregular case is where the argmin set is non-singlton after Theorem 1. 


\item[3.a] \textit{\textcolor{blue}{ The under-coverage performance of $\mbox{CB}_{\alpha,n}$     in small samples (for some
$\omega$) makes me wonder if you could focus on $\mbox{CB}_{\alpha,n,\Measures}$ in the interest of
reducing the length of the paper. }}

 \smallskip

\textbf{Response:} I am using point-wise valid $\mbox{CB}_{\alpha,n}$ as reference for   exact confidence intervals. I would like to keep it in the paper.


\item[3.b] \textit{\textcolor{blue}{  The author responded to my comment regarding the sensitivity analysis (Section 4.3). The simulations, however, are thin and limited.
In my opinion, simulation studies are crucial in assessing the performance
of statistical procedures, especially in nonstandard settings
and especially in the absence of theoretical guidance. In order to
fairly examine the issue, I think it is important to try (i) different
simulation designs, (ii) different sample sizes, and (iii) most importantly
different pairs $\mu_n,\kappa_n$ with $\kappa_n>\mu_n$ (for $\mbox{CB}_{\alpha,n,\Measures}$ as predicted
by the theory). Right now, it is just one design, one sample size, and
only one pair $\mu_n,\kappa_n$ with $\kappa_n>\mu_n$. }}

 \smallskip

\textbf{Response:} There must be some misunderstanding. The uniformly valid bounds $\mbox{CB}_{\alpha,n,\Measures}$ do not depend on the sequence $\kappa_n$. Only $\mbox{CB}_{\alpha,n}$ depends on $\kappa_n$, which the referee recommended to omit in his/her point 3.a.  Moreover, after the last revision, I omitted the requirement $\kappa_n>\mu_n$ for point-wise validity of $\mbox{CB}_{\alpha,n}$ (see Theorem 4 in Appendix B). Figures 8-11 in Appendix D have the results for two additional sequences $\kappa_n$. Finally, Figure 2 shows how two different sample sizes affect coverage  for both $\mbox{CB}_{\alpha,n}$ and $\mbox{CB}_{\alpha,n,\Measures}$. The multiple designs are indexed by $\omega$ and $d$.

The contribution of the paper is the large-sample theory. I believe, the current MC results illustrate all the theoretical results in the paper.  I would like to write a separate follow-up study of the regularization in small samples with particular proposals for tuning parameters. 


\end{enumerate}

==> workPlan.tex <==
\newpage
 
\begin{enumerate}


\item Try the following idea. USe standard deviation of the Minimum as   Noise of for $ \mu$
\end{enumerate}

Last edit here: \pageref{starthere}

\listoftodos


%\listofmycr 


 
